A Survey of JSON-compatible Binary Serialization Specifications

In this paper, we present the recent advances that highlight the characteristics of JSON-compatible binary serialization specifications. We motivate the discussion by covering the history and evolution of binary serialization specifications across the years starting from 1960s to 2000s and onwards. We analyze the use cases of the most popular serialization specifications across the industries. Drawing on the schema-driven (ASN.1, Apache Avro, Microsoft Bond, Cap'n Proto, FlatBuffers, Protocol Buffers, and Apache Thrift) and schema-less (BSON, CBOR, FlexBuffers, MessagePack, Smile, and UBJSON) JSON-compatible binary serialization specifications, we compare and contrast their inner workings through our analysis. We explore a set of non-standardized binary integer encoding techniques (ZigZag integer encoding and Little Endian Base 128 variable-length integer encoding) that are essential to understand the various JSON-compatible binary serialization specifications. We systematically discuss the history, the characteristics, and the serialization processes of the selection of schema-driven and schema-less binary serialization specifications and we identify the challenges associated with schema evolution in the context of binary serialization. Through reflective exercise, we explain our observations of the selection of JSON-compatible binary serialization specifications. This paper aims to guide the reader to make informed decisions on the choice between schema-driven or schema-less JSON-compatible binary serialization specifications.

==> sections/acknowledgments.tex <==
In no particular order, many thanks to Wouter van Oortmerssen, Alessandro
  Triglia, and Christopher Warrington for helpful discussions. Many thanks to
  OSS Nokalva \footnote{\url{https://www.ossnokalva.com}} for offering access
  to and help for using their proprietary ASN-1Step ASN.1 \cite{asn1}
  implementation and IDE.


==> sections/schema-driven-intro.tex <==
In this section, \we discuss the history and characteristics of JSON-compatible
schema-driven binary serialization specifications: ASN.1 PER Unaligned
\cite{asn1-per}, Apache Avro \cite{avro}, Microsoft Bond \cite{microsoft-bond},
Cap'n Proto \cite{capnproto}, FlatBuffers \cite{flatbuffers}, Protocol Buffers
\cite{protocolbuffers} and Apache Thrift \cite{slee2007thrift}.

